A Relative Church-Turing-Deutsch Thesis from Special Relativity and Undecidability

Beginning with Turing's seminal work in 1950, artificial intelligence proposes that consciousness can be simulated by a Turing machine. This implies a potential theory of everything where the universe is a simulation on a computer, which begs the question of whether we can prove we exist in a simulation. In this work, we construct a relative model of computation where a computable \textit{local} machine is simulated by a \textit{global}, classical Turing machine. We show that the problem of the local machine computing \textbf{simulation properties} of its global simulator is undecidable in the same sense as the Halting problem. Then, we show that computing the time, space, or error accumulated by the global simulator are simulation properties and therefore are undecidable. These simulation properties give rise to special relativistic effects in the relative model which we use to construct a relative Church-Turing-Deutsch thesis where a global, classical Turing machine computes quantum mechanics for a local machine with the same constant-time local computational complexity as experienced in our universe.

==> declarations_scrap.tex <==
\section*{Declarations}

Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

\begin{itemize}
\item Funding
\item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
\item Ethics approval 
\item Consent to participate
\item Consent for publication
\item Availability of data and materials
\item Code availability 
\item Authors' contributions
\end{itemize}

\noindent
If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

%%===================================================%%
%% For presentation purpose, we have included        %%
%% \bigskip command. please ignore this.             %%
%%===================================================%%
\bigskip
\begin{flushleft}%
Editorial Policies for:

\bigskip\noindent
Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

\bigskip\noindent
Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

\bigskip\noindent
\textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

\bigskip\noindent
BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
\end{flushleft}

==> old_sections.tex <==
Turing machines provide a fully local description of computation. On top of the spacial non-locality of quantum mechanics through entanglement, there also appears to be a computational non-locality, i.e., the computation is performed outside of our universe. To see how this can be, consider the computation of the time-evolution $\tau$ of a quantum state $\vert\psi(\tau)\rangle$. To compute the quantum state $\vert\psi(\tau)\rangle$ at any time $\tau$, we compute the Schrödinger equation,
\begin{align}
    \vert\psi(\tau + d\tau)\rangle = e^{\frac{-i}{\hbar}\hat{H}(\tau + d\tau)}\vert \psi(0)\rangle = \sum_{j = 0}^{\infty}\frac{(-i (\tau + d\tau)/\hbar)^j}{j!}\hat{H}^j\vert \psi(0)\rangle \label{eq:schrodinger_eq1}
\end{align} where the Hamiltonian $\hat{H}$ has at least $\Omega(4^n)$ elements. Computing (\ref{eq:schrodinger_eq1}) can be greatly simplified if the Hamiltonian has a nice structure. But, in the worst case, the computation will require $\Omega(4^n)$ classical computations. However, nature can compute this operation in only $d\tau$ time. Additionally, the nature of the quantum state is that each element in the vector is a possible measurement of the system, and we only have access to the measurement that the state collapses to. That means the amplitudes of all possible measurements exist \textit{somewhere} and the computation in the Hilbert space is performed \textit{somehow} but we only have access to the collapsed measurement. In this work, we provide a classical description of this computation that preserves the exponential computation in $d\tau$ time 


a matrix multiplication in an exponentially large Hilbert space that either requires an exponentially large space and number of computations $t$, i.e., $\frac{\partial t}{\partial \tau} = \Omega (2^n)$, where $n$ is the number of qubits in your quantum state $\vert\psi(\tau)\rangle$. By claiming that this computation is an axiomatic law of the universe, we neglect the exponential number of operations required for it to occur. However, we need a model that can account for the exponential number of operations required to compute quantum mechanics and the exponential speed-up we experience with respect to the universe's time $\tau$.

\subsubsection{Philosophy of Physics}
  Quantum computing's main advantage is that quantum mechanics can outperform classical computers. However, in this work we show that it is still possible to obtain the exponential advantage seen by quantum mechanics and construct a classical simulation model of the universe that preserves quantum supremacy through special relativistic effects.
\subsubsection{Artificial Intelligence}
Another implication of 

%The main motivation behind artificial intelligence is to construct an A.I. that is conscious or outperforms human consciousness in certain tasks. 

%If we can accomplish this feat of creating a conscious machine, then our own unique existence will come into question.  Though, we don't yet have a mathematical description of consciousness, we are seeing A.I. that are beginning to appear conscious. However, supposing A.I. does develop into conscious beings, several are concerned with the ramifications. 
%The $20^\text{th}$ century saw the birth of several scientific revolutions, including computer science \cite{Turing1937OnEntscheidungsproblem}, artificial intelligence\cite{Turing1950ComputingTuring}, quantum mechanics \cite{Schrodinger1926QuantisierungMitteilung} and relativity \cite{Einstein1905OnKorper,Einstein1916DieRelativitatstheorie}. Half a century after Turing's original work, Benioff, Feynman and Manin put the extended Church-Turing thesis in jeopardy by first providing a quantum mechanical description of a Turing machine \cite{Benioff1980TheMachines} and then noticing that certain quantum mechanical systems could not be efficiently simulated by Turing machines \cite{ Feynman1982SimulatingComputers, Manin1980VychislimoeRussian}. Extending their ideas, Deutsch showed that all physical systems can be simulated efficiently by a quantum Turing machine, otherwise known as the Church-Turing-Deutsch Principle \cite{Deutsch1985QUANTUMCOMPUTER.}. The quantum computing community has come to accept the Church-Turing-Deutsch Principle, and as a result many believe that if we have access to a quantum computer, we can simulated any physical system in the universe to an arbitrary accuracy. 

%Implicitly, these ideas assume that quantum mechanics is an axiom of the universe, an irreducible computational step that would take an exponential amount of time to perform classically. Attempting to simulate quantum mechanics using classical operations would take an exponential amount of time and space to perform the computation. However, the universe seems to do so in a linear amount of time. But, by making quantum mechanics an irreducible computation of the universe, we are neglecting the facts that a) computing quantum mechanics requires an exponential number of exchanges of information to perform and b) the information to describe a quantum state must exist \textit{somewhere}, even if that information is destroyed upon measurement.

%In this work, we resolve the paradox between the computational speed of quantum mechanics and the required number of irreducible operations by constructing a \textit{relative} model of computation that imparts the time dilation and length contraction effects found in Einstein's special relativity \cite{Einstein1905OnKorper}. Just as special relativity assumes a constant speed of light $c$, our relative model assumes a global clock with which all computations are measured. A base Turing machine simulates another machine encoded on its tape. The simulated machine can query any computable function from the base machine before its next state update. This is similar to how the oracle model of computation works, with the differences discussed in Appendix \ref{app:oracles}. The relativistic effects occur when the state and tape of the simulated machine does not change while the base machine is computing the queried function and so the simulated machine cannot record the passage of time or space resources required for the computation. More specifically, the problem of computing the time and space resources used by the base Turing machine is undecidable in the same sense as the Halting problem, and so only the local time and space resources belonging to the simulated machine are decidable. Using these results, we construct a relative Church-Turing-Deutsch thesis by showing how the relativistic effects constructed by the undecidability results can preserve the exponential speed-up seen by quantum mechanics.

\section{Background}
\subsection{Motivation from Simulating Artificial Intelligence}
 Consider a computer scientist Alan simulating a machine, say an artificial intelligence (AI), by hand on a piece of paper. Like all machines, the AI begins in some state $S_0 \in \{0,1\}^n$ encoded with bits on a log sheet and there are a set of rules $\delta$ that will give the next state of the AI $S_{\tau+1}\in \{0,1\}^n$ given the current state $S_{\tau}\in \{0,1\}^n$, i.e., $\delta : S_{\tau} \rightarrow S_{\tau+1}$. A log sheet is given to Alan to write down the state of the AI after following one iteration of the given rules. Sitting next to Alan is a clock keeping track of the amount of time $t$ it takes him to update the AI to its next state. Off to the side he has some scrap paper to assist him so he doesn't need to write on the log-sheet itself. Now, suppose the first few rules are easy and he takes only $1$ minute to compute the AI's first state $S_1$. From state $S_1$, computing $S_2$ is a bit more involved but he is able to compute it in only $5$ minutes. You can imagine that depending on the rule set given to Alan and the current state of the AI, it will take more or less time to compute its next state. The AI's purpose could be arbitrary, but due to Turing we know that the AI can compute any computable function \cite{Turing1937OnEntscheidungsproblem}. In this work, we consider the question of whether the AI can learn the time $t$ or space on the scrap paper it takes for Alan to update its state using $\delta$? Well, we can imagine a scenario where one of the AI rules is ``Write down the time it takes to compute this rule in the state of the AI.'' But, outside of this kind of rule, we will show that it is impossible. Even more interesting, let's suppose \textbf{you} are the AI that Alan is simulating. He is simulating your consciousness and how you interact with the world around you on a piece of paper. For simplicity, let's say it takes one year of time $t$ to compute your brain state from $S_0$ to $S_1$. And then it takes two years to go from $S_1$ to $S_2$. In between that time, the state of your brain is held constant. The question is, does your brain perceive the year long computation time required to go from $S_0$ to $S_1$? What about the two years from $S_1$ to $S_2$? In this work, we prove that it is impossible any machine to compute the time, space, or the error incurred for their simulation. To do so, we formalize the problem using Turing machines.

\subsection{Turing Machine}
 Rather than doing everything by hand on paper, Alan creates a Turing machine $M$ to compute the next state of the AI. A Turing machine is a finite state machine with state set $Q$ acting on an infinite tape of cells with a symbol written in each cell. The Turing machine has a head that can read and write one symbol at a time from an alphabet of symbols $\Gamma$. The machine makes decisions based on the current symbol underneath its head position and its current state by following a transition function $\delta$. Specifically, one time step $t$ for the transition function will dictate the machine to: (1) read/write the symbol underneath the head with a new symbol from $\Gamma$, (2) change its state with another state in $Q$ and (3) move to the left or right, i.e., $\delta : \Gamma \times Q  \nrightarrow \Gamma \times Q \times \{L, R\}$. For shorthand notation, we can equivalently assume that $\delta$ is a function from the tape and machine state at time $t$ to $t+1$, i.e., $\delta : \Gamma^* \times Q \rightarrow \Gamma^* \times Q$, while still obeying the head positioning. We denote a Turing machine by $TM(\delta, Q, \Gamma)$. 
 
 In the context of decidability, Turing machines possess ACCEPT or REJECT states, i.e., $\text{ACCEPT},\text{REJECT} \in Q$. Essentially, a Turing machine is constructed to compute whether a given string $S'$ belongs to a set of strings known as a Language $L$. If the Turing machine accepts, that means it has decided that a string belongs to the language and it enters the ACCEPT state, i.e., $\text{ACCEPT} \in Q$, otherwise, assuming it does not loop forever, it rejects and enters the REJECT state. In Turing's historical paper, he provided a proof that no Turing machine can decide whether another Turing machine encoded in a string on its tape will stop execution or go on forever, otherwise known as the Halting problem. In this paper, we will construct similar undecidable languages to the Halting problem that lay the foundation for a relative Church-Turing-Deutsch thesis. For more information on decidability and Turing machines, we refer the reader to \cite{Arora2009ComputationalApproach,Hopcroft2001IntroductionEdition}. Next, we provide intuition on time dilation and length contraction from special relativity to better understand the effects of our relative model.
 
 %\subsection{Simulation Theory}
 %There is a ``Theory of Everything" that our universe exists in a simulation. This theory is explored heavily throughout pop culture in movies like the Matrix trilogy. Many have discounted this theory for several reasons, but a main reason is that such a theory does not account for computing quantum mechanics. For a simulation theory to construct our current understanding of the universe, it must sufficiently account for the following:
 %\begin{enumerate}
 %    \item The apparent computational efficiency and mathematical accuracy of the physical laws.
 %    \item The smoothness of the physical laws.
 %    \item Our inability to perceive the simulation requirements.
 %    \item The Turing completeness of the laws.
 %\end{enumerate}

%Even if a simulation theory were to achieve all of these conditions, this work shows that proving such a theory is undecidable without the assistance of the machine simulating the universe. 


  %While Turing machines affect one bit of information at a time, quantum mechanics seems to affect an exponential number of bits stored in its \textbf{quantum state} at any given time. Consider a system of $n$ electrons all stationary and equally spaced horizontally in a row. Let's define our \textbf{z-axis} to be up and down, perpendicular to the line along the row of the electrons. One useful quantum mechanical property of electrons are their spin. We can think of the spin of an electron as a vector that either points up $\uparrow$ or down $\downarrow$ along the z-axis, but nowhere in between. Suppose we allow the electrons to randomly choose amongst themselves the orientation of their spins. We can imagine that there will be a random assortment of electrons whose spin points up and points down. We can represent a chosen configuration of spins using the common bra-ket notation of Dirac. For example, if all electrons have chosen spin up, then we represent the configuration as $\vert\uparrow  \uparrow \uparrow \uparrow...\uparrow \rangle$. Suppose we wrote down all of the ways for the electrons to choose their spins. We would have an exponentially large table of $2^n$ configurations. Now, suppose we pick out a subset of those $2^n$ configurations and we want to engineer our system so that the electrons appear in a configuration $\psi_i \in \{\uparrow, \downarrow\}^n$ with an assigned probability $p_i$. Now, simply storing these $2^n$ configurations will take an exponential amount of time in the worst case. But, the amazing thing is that the universe can prepare these probability distributions involving an exponential number of bits for us in only a polynomial number electron interactions. This is the power behind quantum computing. 
  
  %On the surface, this seems to disobey basic causality. However, in this paper we provide a computational prophet model that gives us the computational power of quantum mechanics we desire \textbf{and} does not violate our intuitions. Namely, we propose that the universe is simulated by a Turing machine \textbf{in-between} the time steps of our universe and prove that it is impossible to perceive the exponential computational overhead seen by our simulator.
 %You don't have enough operations to even interact with all of the numbers you're constructing. This leaves us with a few explanations. The first one that many scientists believe is that quantum mechanics is a fundamental axiom of our universe that disobeys our intuition of causality. This idea is perplexing and leaves us with cognitive dissonance, but it seems to not violate information theory so long as we keep the measurement postulate of quantum mechanics. Alternatively, there may be a representation of quantum mechanics which does not require an exponential number of probabilities to keep track of. Much like how a change of basis with the Fourier transform makes signal processing a feasible task in the frequency domain, a change of representation of quantum mechanics may make it computable on classical computers. 
 \subsection{Special Relativity}
 The key component of special relativity is that the speed of light $c$ is constant for all observers in all inertial frames. If the relative velocity $v$ between two observers is constant, then there exists a Lorentz transformation between the space-time coordinates of both observers such that the perception of time and length is different for both observers in order to preserve the speed of light. For simplicity, we assume only a relative velocity in the $x$-direction. From the Lorentz transformation we can derive a Lorentz factor 
 \begin{equation}
     \gamma = \frac{1}{\sqrt{1-\frac{v^2}{c^2}}}.
 \end{equation}
 The Lorentz factor is the ratio between perceived time and length in the direction of the relative velocity. For example, consider a stationary observer Alan standing on a train platform watching Joan go by on a train with velocity of $0.9c$ in the x-direction. The Lorentz factor for this situation is $1/\sqrt{0.19}$ which correlates to Joan experiencing time as going $\sqrt{0.19}$ the rate of Alan's, otherwise known as \textbf{time dilation}. Additionally, Alan sees Joan's length in the x-direction shrink by the same ratio, otherwise known as \textbf{length contraction}. Next, we will construct a relative model which experiences similar effects to time dilation and length contraction from the frame of the simulated machine.

==> scrap.tex <==

\begin{table}[h]
\centering
\begin{tabular}{cc}
Probability    & Configuration                                                      \\ \hline
\multicolumn{1}{|c|}{$p_1$}     & \multicolumn{1}{c|}{$\vert\uparrow \uparrow...\uparrow \rangle$}       \\ \hline
\multicolumn{1}{|c|}{$p_2$}     & \multicolumn{1}{c|}{$\vert\downarrow \uparrow...\uparrow \rangle$}     \\ \hline
\multicolumn{1}{|c|}{$\vdots$}  & \multicolumn{1}{c|}{$\vdots$}                                      \\ \hline
\multicolumn{1}{|c|}{$p_{2^n}$} & \multicolumn{1}{c|}{$\vert\downarrow \downarrow...\downarrow \rangle$} \\ \hline
\end{tabular}
\caption{Electron Spin Configuration Probabilities}
\label{tab:electron_spins}
\end{table}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


